GlORIE-SLAM: Globally Optimized RGB-only Implicit Encoding Point Cloud SLAM

Recent advancements in RGB-only dense Simultaneous Localization and Mapping (SLAM) have predominantly utilized grid-based neural implicit encodings and/or struggle to efficiently realize global map and pose consistency. To this end, we propose an efficient RGB-only dense SLAM system using a flexible neural point cloud scene representation that adapts to keyframe poses and depth updates, without needing costly backpropagation. Another critical challenge of RGB-only SLAM is the lack of geometric priors. To alleviate this issue, with the aid of a monocular depth estimator, we introduce a novel DSPO layer for bundle adjustment which optimizes the pose and depth of keyframes along with the scale of the monocular depth. Finally, our system benefits from loop closure and online global bundle adjustment and performs either better or competitive to existing dense neural RGB SLAM methods in tracking, mapping and rendering accuracy on the Replica, TUM-RGBD and ScanNet datasets. The source code is available at https://github.com/zhangganlin/GlOIRE-SLAM

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage{amssymb}
\usepackage[dvipsnames]{xcolor}
\usepackage{tabularx}
\usepackage{multirow} % used by tables
\usepackage{makecell} % used by tables
\usepackage{colortbl} % used by tables
\usepackage[Export]{adjustbox} % provides valign of images and align
%\usepackage[subrefformat=parens,labelformat=parens]{subcaption} % provides subfigure
\usepackage{arydshln} % dashed lines in tables

\usepackage{pifont} % for checkmark symbols
\usepackage{tikz} % frame around image

% define abbreviations
\def\eg{\emph{e.g.}\xspace} \def\Eg{\emph{E.g.}\xspace}
\def\ie{\emph{i.e.}\xspace} \def\Ie{\emph{I.e.}\xspace}
\def\etc{\emph{etc.}\xspace}
\def\wrt{w.r.t.}
\def\etal{\emph{et al.}\xspace}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\noo}{\textcolor{red}{\xmark}}
\newcommand{\yes}{\textcolor{OliveGreen}{\checkmark}}

% define commands
\newcommand{\ours}{Loopy-SLAM\xspace}
\newcommand{\boldparagraph}[1]{\vspace{0.1em}\noindent{\bf #1}}

% ToDo and Name commands
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
\newcommand{\erik}[1]{\textcolor{blue}{\textbf{Erik:} #1}}
\newcommand{\mo}[1]{\textcolor{purple}{\textbf{Martin:} #1}}
\newcommand{\vlad}[1]{\textcolor{green}{\textbf{Vladimir:} #1}}
\newcommand{\lore}[1]{\textcolor{red}{\textbf{Lorenzo:} #1}}

% green-lightgreen-yellow-white
\colorlet{colorFst}{Green!25}       % first
\colorlet{colorSnd}{SpringGreen!45} % second
\colorlet{colorTrd}{Yellow!30}      % third
\colorlet{colorLow}{darkgray!30}    % low-light color
\colorlet{colorGT}{gray!30}         % GT color
\newcommand{\fs}{\cellcolor{colorFst}\bf}   % first
\newcommand{\nd}{\cellcolor{colorSnd}}      % second
\newcommand{\rd}{\cellcolor{colorTrd}}      % third
\newcommand{\lo}{\color{colorLow}}
\newcommand{\gt}{\cellcolor{colorGT}}      % GT


% moderately tighter setting for spacing between figures, tables and their captions
\setlength{\abovecaptionskip}{3pt plus 3pt minus 3pt} 
\setlength{\belowcaptionskip}{-6pt plus 3pt} 
\setlength{\abovedisplayskip}{0pt}
\setlength{\belowdisplayskip}{0pt}
\setlength\abovedisplayshortskip{0pt}
\setlength\belowdisplayshortskip{0pt}
